On the Use of RBF Interpolation for Flux Reconstruction

Flux reconstruction provides a framework for solving partial differential equations in which functions are discontinuously approximated within elements. Typically, this is done by using polynomials. Here, the use of radial basis functions as a methods for underlying functional approximation is explored in one dimension, using both analytical and numerical methods. At some mesh densities, RBF flux reconstruction is found to outperform polynomial flux reconstruction, and this range of mesh densities becomes finer as the width of the RBF interpolator is increased. A method which avoids the poor conditioning of flat RBFs is used to test a wide range of basis shapes, and at very small values, the polynomial behaviour is recovered. Changing the location of the solution points is found to have an effect similar to that in polynomial FR, with the Gauss--Legendre points being the most effective. Altering the location of the functional centres is found to have only a very small effect on performance. Similar behaviours are determined for the non-linear Burgers' equation.

==> LinearAdvectionDiffusion.tex <==
\section{Linear Advection and Advection Diffusion\label{sec:linearadvdiff}}

In order to perform a series of numerical experiments, two test cases have been chosen --- the linear advection of a sine wave, on a domain $\Omega = [-\pi,\pi]$, and the linear advection-diffusion of a Gaussian bump, on a domain $\Omega = [-10,10]$, according to the equation:

\begin{align}\label{eq:linearAdvection}
        \px{u}{t} + a \px{u}{x} = D \pxi{2}{u}{x}
\end{align}

For both test cases, the advection speed, $a$, is equal to unity, and for the advection-diffusion problem, the diffusion coefficient, $D$, is set to $0.1$. This coefficient is set to zero for the pure advection of the sine wave. Periodic boundary conditions were used in both cases.

To perform these analyses, an initial condition was specified for both cases:
\begin{subequations}\label{eq:LAD_Initial}
\begin{align}
    \boldsymbol{u}_0 & = \boldsymbol{u}(t=0) = \sin{\boldsymbol{x}} \qquad \text{Sine Wave Advection} \\
    \boldsymbol{u}_0 & = \boldsymbol{u}(t=0) = \exp{\left(-\boldsymbol{x}^2\right)} \qquad \text{Gaussian Bump Advection Diffusion}
\end{align}
\end{subequations}

From these initial conditions, the calculations were advanced in time, and the resulting solutions from the calculation at time $t$, $\boldsymbol{u}^\delta(t)$, are compared with the exact analytical solution, $\boldsymbol{u}(t)$, across the entire domain. The difference between the approximate and analytical solutions is reported as an error vector. A variety of ways of measuring the magnitude of this error exist. Here, the error is reported as an $\mathcal{L}^2$ norm of this vector, \emph{i.e.}:
\begin{equation}
    \|\mathcal{E}\|_2  = \sqrt{\sum^N_{j=1}\sum^{n_s}_{i=1}\left(\mathbf{u}^\delta_j(x_i) - u(x_{j,i})\right)^2}
\end{equation}
for a case with $N$ elements and with each element composed of $n_s$ solution points. In addition to the $\mathcal{L}^2$ norm, the $\mathcal{L}^1$ and $\mathcal{L}^\infty$ vector norms were also calculated. These were both found to behave similarly to the $\mathcal{L}^2$ norm across all cases, and so they are further reported here.

By making use of these two test cases, the various factors which might influence the performance of radial basis flux reconstruction are explored in this section.

\subsection{Layout of the Solution Points\label{ssec:solnpointlocs}}

The layout of the solution points within the reference cell is known to have an influence on the performance of flux reconstruction [REF]. It is theorised that this effect is likely to be more significant with radial basis interpolation, because the bases themselves are directly dependent on the point location in a way that the polynomials are not. 

\begin{figure}[htbp]
    \centering
        \adjustbox{width=0.6\linewidth, valign=b}{\input{Figs/tikz/InterpolationPoints}}
    \caption{\label{fig:pointLayouts}Distributions of solution point layout within the reference element.}
\end{figure}

\cref{fig:pointLayouts} shows the solution point locations that have been tested here. The Legendre, Lobatto, and Chebyshev points are familiar from polynomial quadrature theory as the locations of the roots of the relevant functions. They have different advantages and disadvantages in terms of function approximation, and the Lobatto points in particular have some advantages in terms of flux reconstruction. As can be seen from the figure, the Lobatto points include the end points. This means that the flux points are collocated with the terminal solution points, avoiding the need for projection to the flux points, and thereby offering a potential saving in compute time. In addition to these three familiar point layouts, two others have been tested --- one, the `internal' uniform points, which are uniformly distributed over the inside of the cell, with half a spacing between the terminal solution points and the flux points, and two, the `full' uniform points, which are uniformly distributed over the entire cell, from flux point to flux point, and sharing the potential computational benefit of collocated flux and solution points with the Lobatto points. 

\begin{figure}[tbhp]
    \centering
    \subfloat[$n=3$.]{\label{fig:n3_gad_locations}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n3_gad_pointLocations}}}
    ~
    \subfloat[$n=4$.]{\label{fig:n4_gad_locations}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n4_gad_pointLocations}}}
    \newline
    \subfloat[$n=5$.]{\label{fig:n5_gad_locations}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n5_gad_pointLocations}}}
    \caption{\label{fig:gad_locations}The effect of point layout on $L_2$ error for linear advection-diffusion of a Gaussian bump.}
\end{figure}

\begin{figure}[tbhp]
    \centering
    \subfloat[$n=3$.]{\label{fig:n3_sa_locations}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n3_sa_pointLocations}}}
    ~
    \subfloat[$n=4$.]{\label{fig:n4_sa_locations}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n4_sa_pointLocations}}}
    \newline
    \subfloat[$n=5$.]{\label{fig:n5_sa_locations}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n5_sa_pointLocations}}}
    \caption{\label{fig:sa_locations}The effect of point layout on $L_2$ error for linear advection of a sine wave.}
\end{figure}

\cref{fig:gad_locations,fig:sa_locations} show the performance of the RBF-FR method using different point locations for a range of mesh spacings. \cref{fig:gad_locations} shows behaviour of the advection diffusion of the Gaussian bump, and~\cref{fig:sa_locations} shows performance on the pure advection of the sine wave, both at a modest shape function value of $\varepsilon=0.5$, and across three solution point numbers, of $n_s = 3$, $4$, and $5$. For comparison, a set of solutions computed with the polynomial bases using the Legendre is supplied. It is immediately clear that, as expected, there is a strong dependence of accuracy on the point layouts, with close to an order of magnitude of error separating the best performing points from the worst performing points. Typically, the full uniform points and the Lobatto points perform least well, and, in general, the Legendre points perform best. For the advection diffusion equation, there is some evidence in \cref{fig:gad_locations} that the better performing solution point layouts are capable of outperforming the polynomial bases on the coarsest meshes, but that this does not hold true as the meshes are refined. The RBF-FR also seems to perform better, relative to the polynomial baseline, with $3$ and $5$ solution points, performing noticeably worse for the $n_s = 4$ case, for both the advection diffusion and pure advection test cases. 

\cref{fig:gad_locations_01,fig:sa_locations_01} show the same runs as \cref{fig:gad_locations,fig:sa_locations}, but with the shape factor of the radial bases reduced from $0.5$ to $0.1$. As would be expected, as the shape factor is reduced towards zero, the performance of the fit follows the polynomial results more closely --- in the flat limit of $\varepsilon = 0$, the Gaussian RBF fit can be shown to be equivalent to a polynomial fit [REF]. In terms of the point locations, similar trends are observed with the wider Gaussian bases --- there is still close to an order of magnitude of difference between the best and worst performing. Again, the functions with collocated solution and flux points (the full uniform and Lobatto points) are seen to perform least effectively, and the Legendre points are again found to be the most effective of those tested. With the advection diffusion of the Gaussian bump, \cref{fig:gad_locations_01}, there is evidence of the best performing point locations outperforming the polynomial fit across the entire range tested. With the pure advection of the sine wave, \cref{fig:sa_locations_01}, the behaviour of RBF-FR is seen to be more complex. There are pronounced peaks and troughs in the error curves, which typically moves the RBF-FR accuracy either side of the polynomial accuracy. Again, the general trend is that RBF-FR is able to outperform the polynomial method on the coarser meshes, but is overtaken as the meshes are refined.

\begin{figure}[tbhp]
    \centering
    \subfloat[$n=3$.]{\label{fig:n3_gad_locations_01}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n3_gad_pointLocations_01}}}
    ~
    \subfloat[$n=4$.]{\label{fig:n4_gad_locations_01}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n4_gad_pointLocations_01}}}
    \newline
    \subfloat[$n=5$.]{\label{fig:n5_gad_locations_01}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n5_gad_pointLocations_01}}}
    \caption{\label{fig:gad_locations_01}The effect of point layout on $L_2$ error for linear advection-diffusion of a Gaussian bump.}
\end{figure}

\begin{figure}[tbhp]
    \centering
    \subfloat[$n=3$.]{\label{fig:n3_sa_locations_01}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n3_sa_pointLocations_01}}}
    ~
    \subfloat[$n=4$.]{\label{fig:n4_sa_locations_01}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n4_sa_pointLocations_01}}}
    \newline
    \subfloat[$n=5$.]{\label{fig:n5_sa_locations_01}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n5_sa_pointLocations_01}}}
    \caption{\label{fig:sa_locations_01}The effect of point layout on $L_2$ error for linear advection of a sine wave.}
\end{figure}

\subsection{Effect of the Shape Function\label{ssec:shapefunction}}

The scale of the shape function, $\varepsilon$, or equivalently, the relative width of the basis, is known to have a significant effect on the performance of RBF interpolation [REF]. In this section, the effect of reducing this scaling parameter is explored on the two test cases. In all of these cases, the best performing point locations from the previous section were used --- the Legendre points. 

\cref{fig:gad_varEpsilon,fig:sa_varEpsilon} show the effect of reducing this parameter on the performance of RBF-FR, again with a polynomial FR curve for comparison, for $n_s = 3$, $4$, and $5$. Generally, the accuracy of the RBF-FR solution improves as the shape parameter is reduced. \cref{fig:gad_varEpsilon}, which shows the error incurred in the evolution of the Gaussian bump under both advection and diffusion, suggests that each of the shape factors are capable of outperforming the polynomial fit at some grid density. Larger values of $\varepsilon$ tend to outperform the polynomial on extremely coarse grids, but as the grid is refined, the polynomial approach overtakes them. As the value of the shape parameter is reduced, the range of mesh densities at which RBF-FR outperforms polynomial FR moves towards finer meshes. By the time a value of $\varepsilon = 0.1$ is reached, the RBF-FR outperforms the polynomial across the entire range of mesh densities tested, with close to a $50\%$ reduction in the error on the finest mesh tested for $n_s = 5$. The other observable trend in general is that as the shape parameter is reduced, the performance becomes increasingly like that of the polynomial FR. 

\cref{fig:sa_varEpsilon} shows the same tests, but for the pure advection of a sine wave. The RBF-FR performs much less competitively here, but similar trends can be observed --- higher values of shape parameter, so narrower radial bases, tend to outperform the polynomial on more coarse meshes, and wider bases tend to outperform the polynomial FR on finer meshes. However, in all of these cases the polynomial FR outperforms RBF-FR for the finest meshes. Despite this, there are large sections of mesh densities in which the RBF-FR is highly competitive with the polynomial FR in terms of $L_2$ error norm. As seen with the advection diffusion of the Gaussian bump, as the shape parameter is reduced, the curves gradually trend towards the baseline polynomial $L_2$ error curve. However, with the baseline Gaussian Radial Basis function, it was not possible to use shape parameters significantly smaller than this, as the condition number of system of equations requiring to be solved to find $\psi(r)$ from $\phi(r)$ in \cref{eq:RBF_AlternantMatrix} grows extremely rapidly, and numerical errors swamp the solution. A method to ameliorate this is covered in detail in SECTION.

\begin{figure}[tbhp]
    \centering
    \subfloat[$n=3$.]{\label{fig:n3_gad_varEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n3_gad_varEpsilon}}}
    ~
    \subfloat[$n=4$.]{\label{fig:n4_gad_varEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n4_gad_varEpsilon}}}
    \newline
    \subfloat[$n=5$.]{\label{fig:n5_gad_varEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n5_gad_varEpsilon}}}
    \caption{\label{fig:gad_varEpsilon}The effect of shape parameter, $\varepsilon$, on $L_2$ error for linear advection-diffusion of a Gaussian bump.}
\end{figure}

\begin{figure}[tbhp]
    \centering
    \subfloat[Three point $L_2$ error, $n=3$, Legendre points.]{\label{fig:n3_sa_varEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n3_sa_varEpsilon}}}
    ~
    \subfloat[Four point $L_2$ error, $n=4$, Legendre points.]{\label{fig:n4_sa_varEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n4_sa_varEpsilon}}}
    \newline
    \subfloat[Five point $L_2$ error, $n=5$, Legendre points.]{\label{fig:n5_sa_varEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n5_sa_varEpsilon}}}
    \caption{\label{fig:sa_varEpsilon}The effect of shape parameter, $\varepsilon$, on $L_2$ error for linear advection of a sine wave.}
\end{figure}

\subsection{Effect of the RBF Centre Locations}

As well as their shape, radial basis functions are also defined by the locations from which the Euclidean distance which gives $r$ is measured --- their centres. In the previous sections, the centres of the bases have been placed at the same location as the solution points. Here, we investigate the effect of separating them.

\cref{fig:gad_cenLocations} shows this, at two different values of shape parameter. The solution points are kept at the Legendre nodes, and the RBF centres are changed from the Legendre nodes to the full uniform and interal uniform distributions. From the plot, it appears that any influence made by moving the RBF centres is marginal, and, as might be expected, this influence reduces even further as the shape parameter decreases and the bases increasingly accurately approximate $\phi(r)=1$. In general, the results shown here for the advection diffusion of the Gaussian bump suggest that there may be a small benefit in using the full uniform point set as the centres, but this effect is again marginal. It is possible that this small benefit is related to the effect of the functional centre locations on the condition number of the alternant matrix, and thus the numerical accuracy of the fit. This is outlined in more detail in \cref{subsec:smallShapeParameters}. The result, however, was not repeated for the pure advection of the sine wave, and due to the marginal nature of the effect seen, further results are omitted here for brevity.

\begin{figure}[tbhp]
    \centering
    \subfloat[Three point $L_2$ error, $n=3$, Legendre points.]{\label{fig:n3_gad_cenLocations}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n3_gad_cenLocations}}}
    ~
    \subfloat[Four point $L_2$ error, $n=4$, Legendre points.]{\label{fig:n4_gad_cenLocations}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n4_gad_cenLocations}}}
    \newline
    \subfloat[Five point $L_2$ error, $n=5$, Legendre points.]{\label{fig:n5_gad_cenLocations}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n5_gad_cenLocations}}}
    \caption{\label{fig:gad_cenLocations}The effect of varying the RBF centre locations on $L_2$ error for linear advection-diffusion of a Gaussian bump.}
\end{figure}


\subsection{Small Values of Shape Parameter \label{subsec:smallShapeParameters}}

So far, it has been shown that the reduction of $L_2$ error with increased mesh density has been shown to trend towards the polynomial case as the shape parameter is reduced towards zero. However, the RBF alternant matrix shown in \cref{eq:RBF_AlternantMatrix} becomes increasingly ill-conditioned as the the shape parameter decreases, becoming equal to the matrix of ones in the limit $\varepsilon \to 0$. \cref{fig:condNumber_RBFDirect} shows this variation in condition number with shape parameter, which is also affected by the location of the centres, related to the mean distance between the functional centres. A general rule-of-thumb is that a for every order of magnitude the condition number increases by, a digit of precision is lost in the solution. This means that the system of equations cannot be reliably solved for for smaller values of shape parameter. However, various sources have pointed out [REF, REF, REF] that it is not the basis itself that is ill-conditioned --- it is merely an intermediate step in calculating it which is to blame.

\begin{figure}[tbhp]
    \centering
    \adjustbox{width=0.6\linewidth, valign=b}{\input{Figs/tikz/conditionNumber_01}}
    \caption{\label{fig:condNumber_RBFDirect}The effect of reducing $\varepsilon$ on alternant matrix condition number when using direct Gaussian RBFs.}
\end{figure}

To this end, various methods have been developed which circumvent this step to allow an effective basis to be produced when using very flat radial bases. Examples of ways that this has been achieved are the Contour-Padé method [REF] and the RBF-QR method [REF]. Here, since the investigation is restricted to Gaussian radial bases, an approach known as the RBF-GA method is used to build the basis functions without the need to directly solve the system of equations arising from the alternant matrix. The details of the approach are omitted for brevity, but it involves expanding the original Gaussian functions into a Taylor series, and then selecting linear combinations which cause most of these terms to cancel out. The result is a new basis which, critically, spans exactly the same space as the original, but which is well conditioned even at very low values of $\varepsilon$.

\cref{fig:condNumber_RBFGA} shows the effect on the condition number of the solution point alternant matrix of calculating the basis via the RBF-GA method, rather than the directly. The same dependence on the mean spacing between the functional centres is observed, but in general the condition number of the alternant is below $10^3$, making it apparent that by side-stepping the use of the alternant matrix, it becomes numerically feasible to use far smaller values of the shape parameter.

\begin{figure}[tbhp]
    \centering
    \adjustbox{width=0.6\linewidth, valign=b}{\input{Figs/tikz/conditionNumber_02}}
    \caption{\label{fig:condNumber_RBFGA}The effect of reducing $\varepsilon$ on alternant matrix condition number when using RBF-GA.}
\end{figure}

\cref{fig:gad_smallEpsilon,fig:sa_smallEpsilon} show the effect that making use of the RBF-GA approach to compute bases has on the mesh density sweep for the two test cases. It is possible to use lower values of $\varepsilon$, but $\varepsilon=0.1$ is repeated with the RBF-GA approach, and is found to give the same results as the direct RBF method for the test cases --- as expected, given that both span the same functional basis space. 

\begin{figure}[tbhp]
    \centering
    \subfloat[Three point $L_2$ error, $n=3$, Legendre points.]{\label{fig:n3_gad_smallEpsilonc}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n3_gad_smallEpsilon}}}
    ~
    \subfloat[Four point $L_2$ error, $n=4$, Legendre points.]{\label{fig:n4_gad_smallEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n4_gad_smallEpsilon}}}
    \newline
    \subfloat[Five point $L_2$ error, $n=5$, Legendre points.]{\label{fig:n5_gad_smallEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n5_gad_smallEpsilon}}}
    \caption{\label{fig:gad_smallEpsilon}The effect of very small shape parameters on $L_2$ error for linear advection-diffusion of a Gaussian bump.}
\end{figure}

\begin{figure}[tbhp]
    \centering
    \subfloat[Three point $L_2$ error, $n=3$, Legendre points.]{\label{fig:n3_sa_smallEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n3_sa_smallEpsilon}}}
    ~
    \subfloat[Four point $L_2$ error, $n=4$, Legendre points.]{\label{fig:n4_sa_smallEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n4_sa_smallEpsilon}}}
    \newline
    \subfloat[Five point $L_2$ error, $n=5$, Legendre points.]{\label{fig:n5_sa_smallEpsilon}\adjustbox{width=0.49\linewidth, valign=b}{\input{Figs/tikz/n5_sa_smallEpsilon}}}
    \caption{\label{fig:sa_smallEpsilon}The effect of very small shape parameters on $L_2$ error for linear advection  of a sine wave.}
\end{figure}

==> method.tex <==

\begin{figure}[tbhp]
    \centering
    \adjustbox{width=0.6\linewidth, valign=b}{\input{Figs/tikz/Gauss_RBF_correction}}
    \caption{\label{fig:my_label}DGFR left correction functions, with a comparison to the $\mathbb{P}_4$ correction.}
\end{figure}


==> tikz/do_not_delete.tex <==
%this directory is for the cached tikz figures, see  https://www.overleaf.com/learn/latex/Questions/I_have_a_lot_of_tikz,_matlab2tikz_or_pgfplots_figures,_so_I'm_getting_a_compilation_timeout._Can_I_externalise_my_figures%3F
